On Universal Sensor Registration

We present a simple approach for sensor registration in target tracking applications. The proposed method uses targets of opportunity and, without making assumptions on their dynamical models, allows simultaneous calibration of multiple three- and two-dimensional sensors. Whereas for two-sensor scenarios only relative registration is possible, in practical cases with three or more sensors unambiguous absolute calibration may be achieved. The derived algorithms are straightforward to implement and do not require tuning of parameters. The performance of the algorithms is tested in a numerical study.

==> algorithm.tex <==
In this section we derive and discuss the algorithm for the estimation of the sensor-specific rotation matrices as defined in~\eqref{Eq:problem:minimization:objective} and~\eqref{Eq:problem:minimization:constraint}. We begin the discussion with the easiest case of two 3D sensors and a single unknown matrix and proceed gradually to the most complex case of an arbitrary number of 2D sensors.

\subsection{Two Three-Dimensional Sensors, Relative Calibration}
Let $S=2$ and assume that both sensors deliver three-dimensional measurements comprising range, azimuth, and elevation data as defined in~\eqref{Eq:problem:sensor:measurement}. Moreover, assume that there are no angular misalignment errors in the second sensor, namely, $A_2=I_{3\times3}$, where $I_{3\times3}$ is the $3\times3$ identity matrix. This setting may also be interpreted as angularly calibrating one sensor relatively to another (possibly also biased) sensor. In this case, the considered problem~\eqref{Eq:problem:minimization:objective}-\eqref{Eq:problem:minimization:constraint} reduces to
\begin{align}\label{Eq:algorithm:minimization:objective:2sensors:3d}
&\min_{A_{1}}\sum_{i=1}^n\norm{A_{1}\ul{p}_{1}^i+\ul{\ell}_{1}-\paren{\ul{p}_{2}^i+\ul{\ell}_{2}}}^2\\\label{Eq:algorithm:minimization:constraint:2sensors:3d}
&{\rm s.t.}\,A_{1}\,{\rm rotation\, matrix}.
\end{align}
This is a standard Wahba's problem~\cite{wahba1965least} which may be solved optimally by a variety of algorithms~\cite{markley1988attitude}. In the sequel, we refer to a routine solving the following formulation of the Wahba's problem
\begin{align}\label{Eq:algorithm:wahba:objective}
&\min_{A}\sum_{i=1}^n\norm{A\ul{x}^i-\ul{y}^i}^2\\\label{Eq:algorithm:wahba:constraint}
&{\rm s.t.}\,A\,{\rm rotation\, matrix},
\end{align}
as $\verb!Wahba!(\{\ul{x}^i\},\{\ul{y}^i\})$.
We may now summarize the algorithm for relative calibration of angular misalignment errors in the case of two three-dimensional, noiseless sensors.
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[tbh]\caption{Relative Calibration of 2 3D Sensors}
%\setlength{\parskip}{-1pt}
\begin{algorithmic}[1]
\REQUIRE{$\set{\ul{m}_{s}^i,\,i=1,\ldots,n},\,s=1,2$.}%
\STATE{Compute $\{\ul{p}_{s}^i,\,i=1,\ldots,n\},\,s=1,2$.}\label{alg1:step:1}
\STATE{Compute $\{\ul{\tilde{p}}_{2}^i,\,i=1,\ldots,n\}$ where $\tilde{p}_{2}^i\triangleq\ul{p}_{2}^i+\ul{\ell}_{2}-\ul{\ell}_{1}$.}\label{alg1:step:2} %
\STATE{Compute $A_1=\verb!Wahba!(\{\ul{{p}_{1}}^i\},\{\ul{\tilde{p}_{2}}^i\})$.}\label{alg1:step:3}
\ENSURE{$A_1$.}%
\end{algorithmic}
\label{Alg1:2rdr:3d:relative}
\end{algorithm}
$ $\\
Step $1$ of Alg.~\ref{Alg1:2rdr:3d:relative} is a simple transformation of a measurement comprising range, azimuth, and elevation data into cartesian coordinate system centered at the sensor. Step $2$ is a translation of the vectors defined by the $\mathcal{O}_1$ coordinate system into the one defined by $\mathcal{O}_2$. In the absence of noise, two pairs of measurements suffice to find the required rotation. However, since measurement noise is inevitable, as defined in~\eqref{Eq:problem:sensor:measurement}, we need to modify the above algorithm by computing Step $1$ using noisy data, meaning the resulting sets $\{\ul{p}_{s}^i,\,i=1,\ldots,n\},\,s=1,2$ are noisy approximations of the actual cartesian target positions. Although, in principle, two pairs of measurements will still result in a valid rotation matrix, a larger number of such pairs will be required in order to improve the noise-robustness of the estimate.

\subsection{Two Heterogeneous Sensors, Relative Calibration}
We proceed with the case of $S=2$ sensors where one of the sensors delivers, as before, three-dimensional measurements, and the other  generates two-dimensional data comprising (noisy) azimuth and elevation.
In this setting one cannot apply directly the procedure described in Alg.~\ref{Alg1:2rdr:3d:relative} since the two-dimensional sensor's measurement does not have a unique three-dimensional representation of the target position. To comply with the notation of the previous case we assume that sensor $s=2$ is the bias-free, three-dimensional sensor, while sensor $s=1$ generates two-dimensional data and has an unknown angular misalignment bias captured by the rotation matrix $A_1$.

Although a two-angle measurement does not correspond to a cartesian target position, it is equivalent to a direction vector that can be used to find the desired rotation matrix by modifying the objective~\eqref{Eq:algorithm:minimization:objective:2sensors:3d} as follows

\begin{align}\label{Eq:algorithm:minimization:objective:2sensors:23d}
&\min_{A_{1}}\sum_{i=1}^n\norm{A_{1}\ul{q}_{1}^i-\ul{q}_{2}^i}^2\\\label{Eq:algorithm:minimization:constraint:2sensors:23d}
&{\rm s.t.}\,A_{1}\,{\rm rotation\, matrix},
\end{align}
where
\begin{align}\label{Eq:algorithm:minimization:objective:2sensors:23d:q1}
\ul{q}_{1}^i&\triangleq\frac{\ul{p}_{1}^i}{\|\ul{p}_{1}^i\|}\\\label{Eq:algorithm:minimization:objective:2sensors:23d:q2}
\ul{q}_{2}^i&\triangleq\frac{\ul{\tilde{p}}_{2}^i}{\|\ul{\tilde{p}}_{2}^i\|},
\end{align}
and $\ul{\tilde{p}}_{2}^i=\ul{p}_{2}^i+\ul{\ell}_{2}-\ul{\ell}_{1}$.

In other words, instead of finding the optimal rotation between two sets of measurements, in the present case, we find the optimal rotation between the direction vectors resulting from the two-dimensional sensor data and from the translated versions of the three-dimensional sensor data. The resulting algorithm may now be summarized as follows:
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[tbh]\caption{Relative Calibration of 2 Heterogeneous Sensors}
%\setlength{\parskip}{-1pt}
\begin{algorithmic}[1]
\REQUIRE{$\set{\ul{m}_{s}^i,\,i=1,\ldots,n},\,s=1,2$.}%
\STATE{Compute $\{\ul{q}_{1}^i\triangleq\ul{p}_{1}^i/\|\ul{p}_{1}^i\|,\,i=1,\ldots,n\}$.}\label{alg2:step:1}
\STATE{Compute $\{\ul{p}_{2}^i,\,i=1,\ldots,n\}$.}\label{alg2:step:2}
\STATE{Compute $\{\ul{\tilde{p}}_{2}^i,\,i=1,\ldots,n\}$ where $\tilde{p}_{2}^i\triangleq\ul{p}_{2}^i+\ul{\ell}_{2}-\ul{\ell}_{1}$.}\label{alg2:step:3} %
\STATE{Compute $\{\ul{q}_{2}^i\triangleq\ul{\tilde{p}}_{2}^i/\|\ul{\tilde{p}}_{2}^i\|,\,i=1,\ldots,n\}$.}\label{alg2:step:4}
\STATE{Compute $A_1=\verb!Wahba!(\{\ul{{q}_{1}}^i\},\{\ul{{q}_{2}}^i\})$.}\label{alg2:step:5}
\ENSURE{$A_1$.}%
\end{algorithmic}
\label{Alg2:2rdr:23d:relative}
\end{algorithm}
$ $\\


\subsection{Two Three-Dimensional Sensors, Absolute Calibration}
\begin{align}
&\min_{A,B}\sum_{i=1}^N\norm{Ay_i-Bz_i}^2\\
&{\rm s.t.}\,A,B\,{\rm rotation\, matrices}
\end{align}

\begin{theo}Algorithm~\ref{alg:wahba:pair} converges.
\end{theo}
\begin{proof}It is easy to see that the sequence of values of the objective is non-increasing and bounded from below and, therefore, converges.
\end{proof}

\begin{theo}Algorithm~\ref{alg:wahba:pair} converges to the global minimum.
\end{theo}
\begin{proof}
\end{proof}

\subsection{General Three-Dimensional Case}




\subsection{General Two-Dimensional Case}

\subsection{Discussion} 

==> algorithm_general2dcase.tex <==
After addressing the case of a general number of three-dimensional sensors, as described in Section.~\ref{section:algorithm:General3Dcase}, and also, evolute the two three-dimensional sensors case in order to comply with two-dimensional sensors, we are now ready to evolute the general case of general number of two-dimensional sensors.
The idea is essentially the same as in the case of three-dimensional sensors with the extensions described in Section.~\ref{section:algorithm:Two2Dcase}.
Those extensions, should be applied in each iteration's beginning and ending.
It is important to note that, is this case, where each iteration consists of multiple ``two direction Wahba``, for each pair of sensors, one can add the extensions for each sub-iteration, and not only once for a complete iteration. In this paper, we do not discuss advantages for each method. In the numerical study section we used the extensions only for a complete iteration. The first extension can be found in Lines~\ref{alg7:step:3}-~\ref{alg7:step:5} $($Alg.~\ref{Alg7:Nrdr:2d:absolute}$)$, and the second extension is in Line~\ref{alg7:step:12} $($Alg.~\ref{Alg7:Nrdr:2d:absolute}$)$.
The complete routine is summarized in Alg.~\ref{Alg7:Nrdr:2d:absolute}.


\begin{algorithm}[tbh]\caption{Absolute Calibration of $S$ 2D Sensors}
\begin{algorithmic}[1]
\REQUIRE{$\set{\ul{u}_{s}^i,\,i=1,\ldots,n},\,s=1,2,\ldots,S$.}
\STATE{Initialize ${A}_{s}^0=I_{3\times3},\,s=1,2,\ldots,S$, , $j=1$.}\label{alg7:step1}
\REPEAT\label{alg7:step:2}
\STATE{Compute $\{\ul{\tilde{p}}_{0}^i=\verb!Triangulation!(\ul{u}_{1}^i,\ul{u}_{2}^i,\ldots,\ul{u}_{S}^i),i=1,\ldots,n\}$.}\label{alg7:step:3}
\STATE{Compute $\{\ul{\tilde{m}}_{s}^i\}$ by $\{(\ul{u}_{s}^i,\ul{\tilde{p}}_{0}^i),i=1,\ldots,n,s=1,2,\ldots,S\}$.}\label{alg7:step:4}
\STATE{Compute $\{\ul{p}_{s}^i,\,i=1,\ldots,n\},\,s=1,2,\ldots,S$.}\label{alg7:step:5}
\FOR{$s=2$ \TO $S$} \label{alg7:step:6}
\FOR{$t=1$ \TO $s-1$} \label{alg7:step:7}
\STATE{Compute $\{\ul{\tilde{p}}_{s}^i
\triangleq{A}_{s}^{j-1}\ul{p}_{s}^i+\ul{\ell}_{s}-\ul{\ell}_{t},\,i=1,\ldots,n\}$.}\label{alg7:step:8} %
\STATE{Compute $A_{t}^j=\verb!Wahba!(\{\ul{{p}}_{t}^i\},\{\ul{\tilde{p}}_{s}^i\})$.}\label{alg7:step:9}
\STATE{Compute $\{\ul{\tilde{p}}_{t}^i
\triangleq{A}_{t}^{j}\ul{p}^i_{t}+\ul{\ell}_{t}-\ul{\ell}_{s},\,i=1,\ldots,n\}$}\label{alg7:step:10} %
\STATE{Compute $A_s^j=\verb!Wahba!(\{\ul{{p}}_{s}^i\},\{\ul{\tilde{p}}_{t}^i\})$.}\label{alg7:step:11}
\ENDFOR
\ENDFOR
\STATE{Compute $\{\ul{u}_{s}^i,\,i=1,\ldots,n\},\,s=1,2,\ldots,S$.}\label{alg7:step:12}
\STATE{$j=j+1$}\label{alg7:step:13}
\UNTIL{Stopping criteria are met.}\label{alg7:step:14}
\ENSURE{$A_1,\ldots, A_S$.}%
\end{algorithmic}
\label{Alg7:Nrdr:2d:absolute}
\end{algorithm}



==> algorithm_general2dcase_new.tex <==
After addressing the case of a general number of three-dimensional sensors, as described in Section.~\ref{section:algorithm:General3Dcase}, and also, evolute the two three-dimensional sensors case in order to comply with two-dimensional sensors, we are now ready to evolute the general case of general number of two-dimensional sensors.
The idea is essentially the same as in the case of three-dimensional sensors with the extensions described in Section.~\ref{section:algorithm:Two2Dcase}.
Those extensions, should be applied in each iteration's beginning and ending.
It is important to note that, is this case, where each iteration consists of multiple ``two direction Wahba``, for each pair of sensors, one can add the extensions for each sub-iteration, and not only once for a complete iteration. In this paper, we do not discuss advantages for each method. In the numerical study section we used the extensions only for a complete iteration. The first extension can be found in Line~\ref{alg7:step:3} $($Alg.~\ref{Alg7:Nrdr:2d:absolute}$)$, and the second extension is in Line~\ref{alg7:step:12} $($Alg.~\ref{Alg7:Nrdr:2d:absolute}$)$.
The complete routine is summarized in Alg.~\ref{Alg7:Nrdr:2d:absolute}.


\begin{algorithm}[tbh]\caption{Absolute Calibration of $S$ 2D Sensors}
\begin{algorithmic}[1]
\REQUIRE{$\set{\ul{u}_{s}^i,\,i=1,\ldots,n},\,s=1,2,\ldots,S$.}
\STATE{Initialize ${A}_{s}^0=I_{3\times3},\,s=1,2,\ldots,S$, , $j=1$.}\label{alg7:step1}
\REPEAT\label{alg7:step:2}
\STATE{Compute $\{(\ul{\hat{p}}_{1}^i,\ul{\hat{p}}_{2}^i\ldots,\ul{\hat{p}}_{S}^i)=\verb!Triangulation!(\ul{m}_{1}^i,\ul{m}_{2}^i,\ldots,\ul{m}_{S}^i),i=1,\ldots,n\}$.}\label{alg7:step:3}
%\STATE{Compute $\{\ul{\tilde{m}}_{s}^i\}$ by $\{(\ul{u}_{s}^i,\ul{\tilde{p}}_{0}^i),i=1,\ldots,n,s=1,2,\ldots,S\}$.}\label{alg7:step:4}
%\STATE{Compute $\{\ul{p}_{s}^i,\,i=1,\ldots,n\},\,s=1,2,\ldots,S$.}\label{alg7:step:5}
\FOR{$s=2$ \TO $S$} \label{alg7:step:6}
\FOR{$t=1$ \TO $s-1$} \label{alg7:step:7}
\STATE{Compute $\{\ul{\tilde{p}}_{s}^i
\triangleq{A}_{s}^{j-1}\ul{p}_{s}^i+\ul{\ell}_{s}-\ul{\ell}_{t},\,i=1,\ldots,n\}$.}\label{alg7:step:8} %
\STATE{Compute $A_{t}^j=\verb!Wahba!(\{\ul{{p}}_{t}^i\},\{\ul{\tilde{p}}_{s}^i\})$.}\label{alg7:step:9}
\STATE{Compute $\{\ul{\tilde{p}}_{t}^i
\triangleq{A}_{t}^{j}\ul{p}^i_{t}+\ul{\ell}_{t}-\ul{\ell}_{s},\,i=1,\ldots,n\}$}\label{alg7:step:10} %
\STATE{Compute $A_s^j=\verb!Wahba!(\{\ul{{p}}_{s}^i\},\{\ul{\tilde{p}}_{t}^i\})$.}\label{alg7:step:11}
\ENDFOR
\ENDFOR
\STATE{Compute $\{\ul{m}_{s}^i,\,i=1,\ldots,n\},\,s=1,2,\ldots,S$.}\label{alg7:step:12}
\STATE{$j=j+1$}\label{alg7:step:13}
\UNTIL{Stopping criteria are met.}\label{alg7:step:14}
\ENSURE{$A_1,\ldots, A_S$.}%
\end{algorithmic}
\label{Alg7:Nrdr:2d:absolute}
\end{algorithm}



==> algorithm_two2dcase.tex <==
We proceed with the case of $S=2$ sensors which delivers, two-dimensional data including (noisy) azimuth and elevation.
As we discussed in Section \ref{section:TwoHetrogeneous} two-dimensional sensor's measurement does not have a unique three-dimensional representation of the target position, therefore, one cannot apply directly the procedure described in Alg.~\ref{Alg3:2rdr:3d:absolute}.
On the other hand, the existence of two such sensors, placed in different locations, $\ul{\ell}_s$, gives us the possibility to estimate target position. Here, we use triangulation algorithm in order to get three-dimensional representation of the target, as described in Alg.~\ref{Alg5:2rdr:2d:triangulation}.
In order to distinguish between two-dimensional and three-dimensional samples, we now define the two-dimensional samples as
\begin{align}\label{Eq:problem:set:measurements}
\set{\ul{u}_{s}^i,\,i=1,\ldots,n},\,s=1,\ldots,S.
\end{align}
whereas, the three-dimensional samples will remain
\begin{align}\label{Eq:problem:set:measurements}
\set{\ul{m}_{s}^i,\,i=1,\ldots,n},\,s=1,\ldots,S.
\end{align}.

\begin{algorithm}[tbh]\caption{Triangulation by $S$ 2D Sensors}
%\setlength{\parskip}{-1pt}
\begin{algorithmic}[1]
\REQUIRE{$\set{\ul{m}_{s}^i,\,i=1,\ldots,n},\,s=1,2,\ldots,S$.}
\STATE{Compute $\{\ul{p}_{s}^i,\,i=1,\ldots,n\},\,s=1,2,\ldots,S$.}\label{alg5:step1}
\STATE{Initialize ${A}_{s}^0=I_{3\times3},\,s=1,2,\ldots,S$, , $j=1$.}\label{alg5:step2}
\REPEAT\label{alg5:step:3}
\FOR{$s=2$ \TO $S$} \label{alg5:step:4}
\STATE{Compute $A_s^j=\verb!Wahba!(\{\ul{{p}}_{s}^i\},\{\ul{\tilde{p}}_{t}^i\})$.}\label{alg5:step:9}
\ENDFOR
\STATE{$j=j+1$}\label{alg5:step:10}
\UNTIL{Stopping criteria are met.}\label{alg5:step:11}
\ENSURE{$A_1,\ldots, A_S$.}%
\end{algorithmic}
\label{Alg5:2rdr:2d:triangulation}
\end{algorithm}

Now, we can update Alg.~\ref{Alg3:2rdr:3d:absolute} as follows. We should add two sections to the algorithm. \\
The first extension is at the beginning of each iteration. Three-dimensional sample, $\ul{\tilde{p}}_{0}^i$ , is calculated by applying the triangulation procedure over pair of synchronized two-dimensional samples, $\ul{u}_{1}^i$ and $\ul{u}_{2}^i$. The necessity of the triangulation procedure in only for having a range sample, additional to the original azimuth and elevation ones. This is why, after triangulation is done, we calculate range values for each sensor, and define now the updated measure as $\ul{\tilde{m}}_{s}^i,s=1,2$. Next, we calculate the cartesian three-dimensional sample, $\ul{p}_{s}^i$, from the full spherical three-dimensional updated sample. This is done for every sample in the track $(i=1,\ldots,n)$. This extension is described in Lines~\ref{alg6:step:3}$:$~\ref{alg6:step:5} $($Alg.~\ref{Alg6:2rdr:2d:absolute}$)$ . \\
The second extension is at the end of each iteration. As a preparation for the next iteration, a conversion should be done from the cartesian samples $\ul{\tilde{p}}_{s}^i$ back to two-dimensional spherical samples $\ul{u}_{s}^i$. This extension is described in Line~\ref{alg6:step:10} $($Alg.~\ref{Alg6:2rdr:2d:absolute}$)$.

\begin{algorithm}[tbh]\caption{Absolute Calibration of $2$ 2D Sensors}
\begin{algorithmic}[1]
\REQUIRE{$\set{\ul{u}_{s}^i,\,i=1,\ldots,n},\,s=1,2$.}
\STATE{Initialize ${A}_{1}^0=I_{3\times3}$, ${A}_{2}^0 =I_{3\times3}$, $j=1$.}\label{alg6:step:1}
\REPEAT\label{alg6:step:2}
\STATE{Compute $\{\ul{\tilde{p}}_{0}^i=\verb!Triangulation!(\ul{u}_{1}^i,\ul{u}_{2}^i),i=1,\ldots,n\}$.}\label{alg6:step:3}
\STATE{Compute $\{\ul{\tilde{m}}_{s}^i\}$ by $\{(\ul{u}_{s}^i,\ul{\tilde{p}}_{0}^i),i=1,\ldots,n,s=1,2\}$.}\label{alg6:step:4}
\STATE{Compute $\{\ul{p}_{s}^i,\,i=1,\ldots,n\},\,s=1,2$.}\label{alg6:step:5}
\STATE{Compute $\{\ul{\tilde{p}}_{2}^i
\triangleq{A}_{2}^{j-1}\ul{p}_{2}^i+\ul{\ell}_{2}-\ul{\ell}_{1},\,i=1,\ldots,n\}$.}\label{alg6:step:6} %
\STATE{Compute $A_1^j=\verb!Wahba!(\{\ul{{p}}_{1}^i\},\{\ul{\tilde{p}}_{2}^i\})$.}\label{alg6:step:7}
\STATE{Compute $\{\ul{\tilde{p}}_{1}^i
\triangleq{A}_{1}^{j}\ul{p}_{1}^i+\ul{\ell}_{1}-\ul{\ell}_{2},\,i=1,\ldots,n\}$.}\label{alg6:step:8} %
\STATE{Compute $A_2^j=\verb!Wahba!(\{\ul{{p}}_{2}^i\},\{\ul{\tilde{p}}_{1}^i\})$.}\label{alg6:step:9}
\STATE{Compute $\{\ul{u}_{s}^i,\,i=1,\ldots,n\},\,s=1,2$.}\label{alg6:step:10}
\STATE{$j=j+1$}\label{alg6:step:11}
\UNTIL{Stopping criteria are met.} \label{alg6:step:12}
\ENSURE{$A_1, A_2$.}%
\end{algorithmic}
\label{Alg6:2rdr:2d:absolute}
\end{algorithm}
$ $\\



==> algorithm_two2dcase_new.tex <==
We proceed with the case of $S=2$ two-dimensional sensors which delivers, (noisy) azimuth and elevation.
As we discussed in Section \ref{section:TwoHetrogeneous} two-dimensional sensor's measurement does not have a unique three-dimensional representation of the target position, therefore, one cannot apply directly the procedure described in Alg.~\ref{Alg3:2rdr:3d:absolute}.
However, the existence of two such sensors, placed in different locations, $\ul{\ell}_s$, gives us the possibility of estimating the three-dimensional target position.
$\ul{\hat{p}_0}^i$. Here, we use the triangulation algorithm in order to get three-dimensional representation of the target. The triangulation algorithm described in Appendix.~\ref{appendix:triangulation}. %In order to distinguish between two-dimensional and three-dimensional samples, we now define the two-dimensional samples as
%\begin{align}\label{Eq:problem:set:measurements}
%\set{\ul{u}_{s}^i,\,i=1,\ldots,n},\,s=1,\ldots,S.
%\end{align}
%whereas, the three-dimensional samples will remain
%\begin{align}\label{Eq:problem:set:measurements}
%\set{\ul{m}_{s}^i,\,i=1,\ldots,n},\,s=1,\ldots,S.
%\end{align}.
It is important to mention, that we are using the triangulation algorithm in order to have the range samples, which are absent in the kind of sensors we use. We do not use the triangulation to update the azimuth and elevation samples.
Now, we can update Alg.~\ref{Alg3:2rdr:3d:absolute} as follows. We should add two sections to the algorithm. \\
The first extension is at the beginning of each iteration. We call it the $\verb!Triangulation!$ section. In this section three-dimensional sample, $\ul{\hat{p}}_0^i$ , is calculated by applying the triangulation procedure over pair of synchronized two-dimensional samples, $\ul{m}_{1}^i$ and $\ul{m}_{2}^i$. The necessity of the triangulation procedure in only for having a range sample, additional to the original azimuth and elevation ones. This is why, after triangulation is done, we calculate range values for each sensor, and define now the updated measure as $\ul{\hat{m}}_{s}^i,s=1,2$. Next, we calculate the cartesian three-dimensional sample, $\ul{\hat{p}}_{s}^i$, from the full spherical three-dimensional updated sample. This is done for every sample in the track $(i=1,\ldots,n)$. This extension is described in Line~\ref{alg6:step:3}$($Alg.~\ref{Alg6:2rdr:2d:absolute}$)$ . \\
The second extension is at the end of each iteration. As a preparation for the next iteration, a conversion should be done from the cartesian samples $\ul{p}_{s}^i$ back to two-dimensional spherical samples $\ul{m}_{s}^i$. This extension is described in Line~\ref{alg6:step:10} $($Alg.~\ref{Alg6:2rdr:2d:absolute}$)$.

\begin{algorithm}[tbh]\caption{Absolute Calibration of $2$ 2D Sensors}
\begin{algorithmic}[1]
\REQUIRE{$\set{\ul{u}_{s}^i,\,i=1,\ldots,n},\,s=1,2$.}
\STATE{Initialize ${A}_{1}^0=I_{3\times3}$, ${A}_{2}^0 =I_{3\times3}$, $j=1$.}\label{alg6:step:1}
\REPEAT\label{alg6:step:2}
\STATE{Compute $\{(\ul{\hat{p}}_{1}^i,\ul{\hat{p}}_{2}^i)=\verb!Triangulation!(\ul{m}_{1}^i,\ul{m}_{2}^i),i=1,\ldots,n\}$.}\label{alg6:step:3}
%\STATE{Compute $\{\ul{\tilde{m}}_{s}^i\}$ by $\{(\ul{u}_{s}^i,\ul{\tilde{p}}_{0}^i),i=1,\ldots,n,s=1,2\}$.}\label{alg6:step:4}
%\STATE{Compute $\{\ul{p}_{s}^i,\,i=1,\ldots,n\},\,s=1,2$.}\label{alg6:step:5}
\STATE{Compute $\{\ul{\tilde{p}}_{2}^i
\triangleq{A}_{2}^{j-1}\ul{p}_{2}^i+\ul{\ell}_{2}-\ul{\ell}_{1},\,i=1,\ldots,n\}$.}\label{alg6:step:6} %
\STATE{Compute $A_1^j=\verb!Wahba!(\{\ul{{p}}_{1}^i\},\{\ul{\tilde{p}}_{2}^i\})$.}\label{alg6:step:7}
\STATE{Compute $\{\ul{\tilde{p}}_{1}^i
\triangleq{A}_{1}^{j}\ul{p}_{1}^i+\ul{\ell}_{1}-\ul{\ell}_{2},\,i=1,\ldots,n\}$.}\label{alg6:step:8} %
\STATE{Compute $A_2^j=\verb!Wahba!(\{\ul{{p}}_{2}^i\},\{\ul{\tilde{p}}_{1}^i\})$.}\label{alg6:step:9}
\STATE{Compute $\{\ul{m}_{s}^i,\,i=1,\ldots,n\},\,s=1,2$.}\label{alg6:step:10}
\STATE{$j=j+1$}\label{alg6:step:11}
\UNTIL{Stopping criteria are met.} \label{alg6:step:12}
\ENSURE{$A_1, A_2$.}%
\end{algorithmic}
\label{Alg6:2rdr:2d:absolute}
\end{algorithm}
$ $\\



==> numerical_roni.tex <==
%\section{Numerical Analysis}


\subsection{Simulation Setup}
In order to examine the suggested algorithm, we simulated a 3-D track, which will be issued as
"Ground-Truth".
The track is simulated as a plane ascending at $10$[m/s] in z axis, while in x-y axis has period of const direction velocity of $+100$[m/s] in x axis, period of circular route in which changes its direction for positive x to negative x, then, respectively, period of const direction velocity of $-100$[m/s] in x axis and circular route back again to x axis.
The track takes $30$[min] and is sampled in reacquisition rate of $1/20$Hz, so that we have $ n=91 $ samples from the simulated track - $\set{\ul{p}_0^i,\,i=1,\ldots,n}$ ~\eqref{Eq:problem:set:positions:global}.
In addition, we placed $ S=3-5 $ sensors in the 3-D space, with different distances from the track,
different point of views, and with variety of heights. Sensors' position ${\ell}_s$ will be as declared at ~\eqref{Eq:problem:biased:sensor_positions}.
For each sensor, as was described in ~\eqref{Eq:problem:set:measurements} it's measurements are defined as: $\set{\ul{m}_{s}^i,\,i=1,\ldots,n},\,s=1,\ldots,S$..
Moreover, we defined the sensors' spherical error distribution, as mentioned in ~\eqref{Eq:problem:sensor:measurement} - $n_{r,s}$, $n_{a,s}$, and $n_{e,s}$ as measurement noises in, respectively, range, azimuth and elevation. These are taken to be independent, Gaussian, with zero mean and known variances $\sigma_r^2$, $\sigma_a^2$, and $\sigma_e^2$.
The errors that we took are: $\sigma_a=\sigma_e=5[mRad]$ and $\sigma_r=20[m]$.
It is worth noting that, in the two-dimensional case $\sigma_r$ is not used anywhere.
It is important to note that, although the algorithm results refers to the Ground-Truth,
the convergence condition, also as, all algorithm steps are based only on the input measurements,
not using any external knowledge, as Ground-Truth information.

%%\begin{figure*}[h!t!]\centering
%%\subfloat[]{\includegraphics[width=0.45\textwidth, trim=0cm 0cm 0cm 0cm]{GT_XY_12_03.eps}}\hspace{0.2cm}
%%\subfloat[]{\includegraphics[width=0.45\textwidth, trim=0cm 0cm 0cm 0cm]{GT_XZ_12_03.eps}}%\hspace{0.2cm}
%%\caption{Caption}
%%\label{fig:numerical:2d3d:errors}
%%\end{figure*}


%\begin{figure}
%  \includegraphics[width=\linewidth]{boat.jpg}
%  \caption{A boat.}
%  \label{fig:boat1}
%\end{figure}
%Figure \ref{fig:boat1} shows a boat.

\subsection{Three-Dimensional Case}
Here, we represent numerical results for absolute calibration with $3, 4$ and $5$ three-dimensional sensors.
In this case, as described earlier, we use $Wahba$ Algorithm between all pairs of sensors' measurements (translated to relevant axes), iteratively.
We do this until, the $A_s,s\in\set{1,\ldots,S}$ rotation matrices converges.
Let's declare
\begin{align}
err_{s,t}=\sum_{i=1}^n\norm{A_{s}\ul{p}_{s}^i+\ul{\ell}_{s}-\paren{A_{t}\ul{p}_{t}^i+\ul{\ell}_{t}}}^2
\end{align}
where $s,t\in\set{1,\ldots,S}$ and $s\neq t$. And also,
\begin{align}
err_{total}=\sum_{s=1}^{S}{\sum_{t=1}^{s-1}err_{s,t}}.
\end{align}
Now, our stopping condition is convergence of $err_{total}$. Implicitly, after iteration that $err_{total}$ changes less than $0.1\%$ from it value, we stop.

\subsection{Two-Dimensional Case}
In correspondence to previous paragraph, we calculate $ \tilde{x}_{ij} $
Then, we change the coordinates from cartesian to spherical. In that case we now have:
$ Az_{ij}, El_{ij} $ and $ Range_{ij} $. Because we are simulate 2-D sensor, we must omit
The $Range_{ij}$.

\subsection{Problematic Cases}
Similar to the previous paragraph, we

\subsection{Discussion}
Similar to the previous paragraph, we

\subsubsection{Algorithm Parameters}
In contrast to other algorithms of optimization, such as gradient descent, in our method we do not use any parameters.

\subsubsection{Convergence Rate}
Here we should enter some word about so many things that will make the readers astonished by our work...

\subsubsection{Two-Dimetional Vs Three-Dimentional Accuracy}
Here we should enter some word about so many things that will make the readers astonished by our work...


\begin{table}[h!t!]
\renewcommand{\arraystretch}{1.3}
\caption{Errors vs. Number of 2D Sensors}
\label{table:errors:2d}
\begin{center}
\begin{tabular}{r|c|c|c|c}
\toprule
& \textbf{3 Sensors} & \textbf{5 Sensors} & \textbf{7 Sensors} & \textbf{9 Sensors}\\
\hline
$err_\psi$[mRad]   & $0.85\pm0.41$ & $0.70\pm0.41$ & $0.57\pm0.20$ & $0.47\pm0.17$ \\
\hline
$err_\theta$[mRad] & $0.95\pm0.49$ & $0.80\pm0.36$ & $0.80\pm0.35$ & $0.66\pm0.27$ \\
\hline
$err_\phi$[mRad]   & $2.04\pm1.19$ & $1.55\pm0.73$ & $1.52\pm0.66$ & $1.03\pm0.31$ \\
\hline
$err_{cart}$[m]    & $133.6\pm9.7$ & $114.3\pm6.0$ & $102.6\pm3.4$ & $90.0\pm2.4$ \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

\begin{table}[h!t!]
\renewcommand{\arraystretch}{1.3}
\caption{Errors vs. Number of 3D Sensors}
\label{table:errors:3d}
\begin{center}
\begin{tabular}{r|c|c|c|c}
\toprule
& \textbf{3 Sensors} & \textbf{5 Sensors} & \textbf{7 Sensors} & \textbf{9 Sensors}\\
\hline
$err_\psi$[mRad]   & $0.45\pm0.21$ & $0.43\pm0.15$ & $0.38\pm0.13$ & $0.36\pm0.10$ \\
\hline
$err_\theta$[mRad] & $0.62\pm0.32$ & $0.62\pm0.19$ & $0.60\pm0.19$ & $0.50\pm0.16$ \\
\hline
$err_\phi$[mRad]   & $1.45\pm0.72$ & $1.28\pm0.58$ & $1.01\pm0.36$ & $0.83\pm0.26$ \\
\hline
$err_{cart}$[m]    & $101.0\pm3.9$ &  $96.2\pm2.9$ &  $92.6\pm2.1$ & $83.8\pm1.5$ \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

\begin{figure*}[h!t!]\centering
\subfloat[]{\includegraphics[width=0.45\textwidth, trim=0cm 0cm 0cm 0cm, clip]{test.eps}}\hspace{0.2cm}
\subfloat[]{\includegraphics[width=0.45\textwidth, trim=0cm 0cm 0cm 0cm, clip]{Sum2D3D.eps}}%\hspace{0.2cm}
%\subfloat[]{\includegraphics[width=0.5\textwidth, trim=1cm 0.2cm 1cm 0.5cm, clip]{test.eps}}%\hspace{0.2cm}
\caption{Caption}
\label{fig:numerical:2d3d:errors}
\end{figure*}

\begin{figure*}[h!t!]\centering
\subfloat[]{\includegraphics[width=0.45\textwidth, trim=0cm 0cm 0cm 0cm, clip]{Convergence_N4_3D_noise2.eps}}\hspace{0.2cm}
\subfloat[]{\includegraphics[width=0.45\textwidth, trim=0cm 0cm 0cm 0cm, clip]{Convergence_N4_2D_noise2.eps}}%\hspace{0.2cm}
%\subfloat[]{\includegraphics[width=0.5\textwidth, trim=1cm 0.2cm 1cm 0.5cm, clip]{test.eps}}%\hspace{0.2cm}
\caption{Caption}
\label{fig:numerical:2d3d:errors}
\end{figure*}


\begin{figure*}[h!t!]\centering
\subfloat[]{\includegraphics[width=0.45\textwidth, trim=0cm 0cm 0cm 0cm, clip]{Samples2D.eps}}\hspace{0.2cm}
\subfloat[]{\includegraphics[width=0.45\textwidth, trim=0cm 0cm 0cm 0cm, clip]{Noises2D.eps}}%\hspace{0.2cm}
%\subfloat[]{\includegraphics[width=0.5\textwidth, trim=1cm 0.2cm 1cm 0.5cm, clip]{test.eps}}%\hspace{0.2cm}
\caption{Caption}
\label{fig:numerical:2d3d:errors}
\end{figure*}





